BIGCity: A Universal Spatiotemporal Model for Unified Trajectory and Traffic State Data Analysis

Typical dynamic ST data includes trajectory data (representing individual-level mobility) and traffic state data (representing population-level mobility). Traditional studies often treat trajectory and traffic state data as distinct, independent modalities, each tailored to specific tasks within a single modality. However, real-world applications, such as navigation apps, require joint analysis of trajectory and traffic state data. Treating these data types as two separate domains can lead to suboptimal model performance. Although recent advances in ST data pre-training and ST foundation models aim to develop universal models for ST data analysis, most existing models are "multi-task, solo-data modality" (MTSM), meaning they can handle multiple tasks within either trajectory data or traffic state data, but not both simultaneously. To address this gap, this paper introduces BIGCity, the first multi-task, multi-data modality (MTMD) model for ST data analysis. The model targets two key challenges in designing an MTMD ST model: (1) unifying the representations of different ST data modalities, and (2) unifying heterogeneous ST analysis tasks. To overcome the first challenge, BIGCity introduces a novel ST-unit that represents both trajectories and traffic states in a unified format. Additionally, for the second challenge, BIGCity adopts a tunable large model with ST task-oriented prompt, enabling it to perform a range of heterogeneous tasks without the need for fine-tuning. Extensive experiments on real-world datasets demonstrate that BIGCity achieves state-of-the-art performance across 8 tasks, outperforming 18 baselines. To the best of our knowledge, BIGCity is the first model capable of handling both trajectories and traffic states for diverse heterogeneous tasks. Our code are available at https://github.com/bigscity/BIGCity

==> content/1_introduction.tex <==
\section{\textcolor{red}{Introduction}}

Spatiotemporal (ST) data analysis has long been a prominent area of research in the fields of data mining and machine learning. Classic ST data analysis models include trajectory prediction~\cite{trajectory2vec, Toast, JCLRNT, ma2024more}, classification~\cite{Trembr, jiang2023self}, generation~\cite{yuan2022activity, long2023practical, jiang2023continuous, zhu2024difftraj}, and traffic state prediction models~\cite{wu2020connecting, li2021traffic, deng2021st, guo2023self}, among others~\cite{atluri2018spatio}. 
These models play pivotal roles in numerous intelligent transportation systems (ITS)~\cite{hoteit2014estimating}, smart city initiatives~\cite{chen2021robust, li2022spatial}, and location-based service (LBS) applications~\cite{gao2023predicting}. With the boom of deep learning, deep neural network-based methods have become the mainstream approach for ST data analysis, 
achieving significant success in many practical applications.
% leveraging their ability to model complex data correlations. Numerous specialized deep learning models have been proposed for various ST data analysis tasks, achieving significant success in many practical applications. 
Despite these advancements, current spatiotemporal analysis methods are often narrowly tailored to specific tasks. This limits the models' ability to capture broad patterns and relationships across different tasks, restricting their performance and generalization in real-world applications.

In recent years, universal deep learning models capable of handling multiple tasks with a single model have achieved significant breakthroughs~\cite{zhao2023surveylargelanguagemodels}. Trained on large, diverse datasets, these models demonstrate strong cross-dataset generalization or multi-task versatility, often outperforming task-specific methods in various applications. 
% Notable examples include the GPT series~\cite{radford2019language, brown2020language}, LVM~\cite{bai2023sequentialmodelingenablesscalable}, and CogVLM~\cite{wang2023cogvlm}, which 
Notable examples have demonstrated great success in natural language processing (NLP)~\cite{radford2019language, brown2020language}, computer vision (CV)~\cite{bai2023sequentialmodelingenablesscalable}, and multimedia (MM)~\cite{wang2023cogvlm}. 
However, in ST data analysis, research on unified multi-tasks models is still nascent, with several unique challenges constraining their development, such as the following.

\begin{figure}[t]
     \centering
     \includegraphics[width=0.90\columnwidth, page=1]{figure/1_intro/intro_figure.pdf}
     \caption{\textcolor{red}{Performance Radarchart of \name on Various Tasks.}}
     \label{fig:intro}
\end{figure}

\textbf{(1) Challenges in developing unified representations of ST data:} For NLP applications, all textual data can be uniformly represented as sequence of  characters, while for CV applications, images can be uniformly represented as a matrices or tensors composed of pixels. However, in ST data analysis, the two most important types of data, individual trajectories and collective traffic states, are usually treated as two mutually incompatible data modalities. Trajectory data are considered as sequences of geographical units, such as road segments or points of interest (POI). In contrast, traffic state data are typically represented as graphs with dynamic signals, such as traffic speed over urban road networks. However, for many ST data applications, system needs to handle the two types of data at the same time, for example navigation APPs. How to unify these two different data modalities remains a challenging task.

\textbf{(2) Challenges in unifying heterogeneous ST analysis tasks:} 
In NLP, heterogeneous tasks can be unified as the next-word generation. This enables a single model to efficiently handle various tasks. However, for the ST data, different data analysis tasks are highly heterogeneous. 
On one hand, data formats various from task to task. For example, with the same trajectory inputs, the outputs for the travel time estimation task is continuous time, while for route planning is another trajectory. 
On the other hand, the diverse complexity of heterogeneous tasks demands supervision signals at different levels of granularity, resulting in various training formats.
How to unifying the heterogeneous tasks in the unified format still remains a challenge.

In the literature, early works have adopted representation learning methods to construct versatile ST data representations for various downstream tasks~\cite{balsebre2023cityfm, 10.1145/3394486.3403043, jiang2023self}. Most of these methods focus on individual static geographic elements, such as road networks and points of interest (POI), or solely on trajectories. Another approach involves using specialized models as tools while training a general model to employ these tools. This paradigm creates a universal ST data analysis system rather than a single model~\cite{zhang2023trafficgpt}. 
Here, the general model does not directly interpret ST data, which limits its ability to uncover correlations across diverse tasks. 
Newly emerging models designed solely for traffic state prediction tasks to achieve cross-dataset generalization~\cite{yuan2024unist, li2024urbangpt} or for multiple trajectory-based tasks~\cite{zhou2024plm4trajcognizingmovementpatterns} have achieved impressive performance. However, developing a universal model capable of simultaneously handling both trajectory and traffic state data across heterogeneous tasks remains a significant challenge.


To address those challenges, we propose a {\underline{B}}i-modality {\underline{I}}nteractive {\underline{G}}eneral model for Spatio{\underline{T}}emporal data analysis (\name).
The model is designed to address prevalent spatiotemporal applications based on road networks, including trajectory and traffic state tasks.
For the challenge of unified data representations, the \name expresses ST data from two different modality~(trajectories and traffic state series) into a unified format using the proposed {\em Spatiotemporal (ST) Units}. ST data from both modalities can be expressed as a sequence of ST Units, and further represented as token vectors by the proposed {\em Spatiotemporal Tokenizer}. 
For the challenge of task heterogeneity, we proposed the {\em interactive prompts} to uniformly tokenize the task-specific data across heterogeneous tasks, including input data and task-relevant specifications.
Further, we constructed a {\em hierarchical training strategy} to satisfy the requirements of tasks across various complexity levels. 

Specifically, the proposed interactive prompts consists of: $i$) a textual instruction guiding our model on the type of task to be performed, $ii$) a sequence of input data  (a trajectory or a traffic state series) in the format of ST unit tokens, and $iii$) a sequence of unified task placeholders which informs the output format and are further converted into output results for various heterogeneous tasks.
Additionally, the hierarchical training strategy is composed by three progressive stages:  $i$) a trajectory reconstruction for model pre-training, $ii$) a task-oriented prompt tuning enabling the model task adaptability, and $iii$) a generative reinforcement learning to enhance the model in trajectory generation tasks.

In the experiments, the \name model outperforms 28 baselines across seven tasks over three real-world datasets. Fig \ref{fig:intro} summarizes the versatility of the \name model by using the \xa Dataset.

% The outputs are a sequence of result tokens that can be decoded as different formats according to requirements of target tasks. We adopt a progressive training strategy, including 
%The experimental results show that our method achieves State-of-the-Art performance in five downstream tasks on three real datasets. As illustrated in Fig \ref{fig:intro}, \name demonstrates the comprehensive ability to process various downstream tasks while maintaining competitive performance in each of them.

\eat{
Also, we provide a theoretical argument that states the validity of our method.
Here, we summarize our key contributions as follows:
\begin{itemize}[leftmargin=*]
\item We investigate the problem of establishing a universal model for spatio-temporal trajectory analysis, which is crucial for enhancing the model’s performances and generalization capabilities across diverse trajectory downstream tasks.
\item We devise a fine-tuning methodology tailored to address spatio-temporal trajectory data to capture the universal spatio-temporal trajectory representations for various tasks.
\item We put forward \name, a %pioneering
spatio-temporal trajectory universal model that automatically manages diverse tasks within an integrated model architecture built upon universal representation learning.
\item We demonstrate the effectiveness and universality of our approach in spatio-temporal trajectory analysis through extensive experiments on three real-world datasets.
\end{itemize} 
}

==> content/2_preliminary.tex <==

\section{Preliminaries}
In this section, we first formally define the basic spatiotemporal (ST) elements. Subsequently, we define the types of ST data processed by \name. In the problem statement, we provide definitions of ST tasks. 

\subsection{Basic Spatiotemporal Elements}
\label{basic_ST_element}
In urban scenarios, road segments are the fundamental spatial elements, while time slices and timestamps form the basic temporal elements.
\begin{mydef}[Road Segment]
    For a city map with $N$ roads, let $R$ denotes the set of road segments, where $\mathcal{R} = \{r_1, \ldots, r_n, \ldots, r_N\}$. Each road segment $r_i$ is associated with a static feature $\bm{e}_i^{(s)} \in \mathbb{R}^{D_r}$. Typically, $\bm{e}_i^{(s)}$ includes road ID, road type, length, land count, in-degree, out-degree and maximum speed limit. 
\end{mydef}
\begin{mydef}[Road Network]
    Road network is a direct graph of road segments, which is represented as $\mathcal{G} = \left\{\mathcal{R}, \mathcal{A}, \bm{E}^{(s)}\right\}$. Specifically, $\mathcal{R}$ is the road segments set. $\mathcal{A} \in \mathbb{R}^{|\mathcal{R}|\times|\mathcal{R}|}$ is a binary value adjacency matrix, indicating whether there is a direct link between road segments. $\bm{E}^{(s)}$ is the static feature set of $R$, where $ \bm{E}^{(s)} = \{\bm{e}_1^{(s)}, \ldots, \bm{e}_n^{(s)}, \ldots, \bm{e}_N^{(s)}\}$.   
\end{mydef}
\begin{mydef}[Timestamp and Time Slice]
    A timestamp, denoted as $\tau$, represents a instantaneous UTC time precise to the second. $\bm{\iota}_{\tau} \in \mathbb{R}^{D_\tau}$ is the temporal feature of $\tau$, including the day index within a week, the minute index of a day, and the second; A time slice represents a 30-minute interval, serving as the smallest temporal unit for traffic state data. The dataset is segmented into $T$ slices, with indexes as $\{1, \ldots, t, \ldots, T\}$. Similarly, $\bm{\iota}_{t} \in \mathbb{R}^{D_t}$ is the temporal feature of the $t$-th time slice, corresponding to a UTC time precise to 30 minutes.
\end{mydef}

\subsection{Spatiotemporal Data}
% Spatiotemporal data is composed by individual spatial and temporal elements. There are two types of spatiotemporal data: trajectory and traffic state.
\begin{mydef}[Trajectory]
    Trajectories are micro-level spatiotemporal data related to individual person. A trajectory $\mathcal{T}$ is a time-order sequence of road segments, where $\mathcal{T} = \left [ (r_{(l)}, \tau_{(l)}) \right ]_{l=1}^L$ and $L$ is the length of $\mathcal{T}$.~Specifically, $r_{(l)}$ and $\tau_{(l)}$ represent the road segment index and timestamp of the $l$-th sample in $\mathcal{T}$, respectively.
\end{mydef}

\begin{mydef}[Traffic State]
    Traffic state refers to marco-level spatiotemporal data related to a group of people.
    For a road segment $r_i$, and its traffic state features includes average speed, traffic inflow, and traffic outflow. Let $\bm{e}_{i, t}^{(d)} \in \mathbb{R}^D_t$ denotes the traffic state of $r_i$ in the $t$-th time slice. Further, the traffic state of all road segments $\mathcal{R}$ is a matrix of $\bm{E}_t^{(d)} \in \mathbb{R}^{N \times D_t}$. The historical traffic states during $t-{T}'$ to $t-1$ are expressed as $\mathcal{\bm{E}}_t^{(d)} = \left\{\bm{E}_{t-{T}'}^{(d)}, \cdots, \bm{E}_{t-1}^{(d)} \right\} \in \mathbb{R}^{{T}' \times N \times D_t}$, and $\bm{E}_{t}^{(d)}$ is the one-slice future traffic states of $\mathcal{\bm{E}}_t^{(d)}$.
\end{mydef}


\subsection{Problem Statement}
\label{problem_statement}
\name processes heterogeneous ST data, including trajectories $\mathcal{T}$ and historical traffic states $\mathcal{E}_t^{(d)}$. First, $\mathcal{T}$ and $\mathcal{E}_t^{(d)}$ are convert into the unified representations as ${\mathcal{U}}$ (in section~\ref{stunit}). Next, \name addresses heterogeneous ST tasks guided by task-specific instructions $\mathcal{I}$ (in section~\ref{sec:tunable_LLM_backbone}). Therefore, we define ST analysis tasks as:
\begin{equation}
    y = f({\mathcal{U}},\mathcal{I};\Theta) .
\end{equation}
where $f(\cdot, \cdot)$ represent \name model and $\Theta$ is the parameters to learn. $y$ represents task results, with its format varies depending on the task type. Specifically, we conclude ST tasks into four categories: $1)$ {\em Classification}, \ie next hop prediction and trajectory classification $2)$ {\em Regression}, \ie travel time estimation (ETA) and traffic state regression $3)$ {\em Generation}, \ie trajectory recovery. $4)$ {\em Comparison}, \ie the most similar trajectory search.



==> content/3_1_overall_framework.tex <==
\section{The Overall Framework}
\name is designed to process heterogeneous ST data and tackle diverse ST tasks. As shown in Figure~\ref{fig:model_architecture}, it comprises two core components: a spatiotemporal tokenizer (in section~\ref{stunit}) and a tunable large language model (LLM) backbone (in section~\ref{model_structure}).

The spatiotemporal tokenizer addresses the heterogeneity in ST data. It encodes both sequence-based trajectories and graph-based traffic states into unified representation format. The tunable LLM backbone, guided by the task-oriented prompt mechanism, enables \name to tackle diverse ST tasks with huge differences.

In the section~\ref{sec:training}, we introduce the training process of \name. First, \name undergoes masked reconstruction training to capture general ST data features. Then, task-oriented prompt training is employed to equip \name with multi-task capabilities.



==> content/3_2_ST_tokenizer.tex <==

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/2_preliminary/STUnit.pdf}
    \caption{\textcolor{red}{A unified expression for spatiotemporal data}}\label{STUnit}
\end{figure}

\section{The Spatiotemporal Tokenizer}

Analogous to how a dictionary provides basic words in natural NLP, the spatiotemporal tokenizer serves as a library of ST features, thereby offering unified representations for heterogeneous ST data. As ST data can be viewed as combinations of basic ST elements, despite their various structures and semantics.

Specifically, we first introduce the concept of {\em unified spatiotemporal (ST) units}, which standardize the data format for ST data. Subsequently, we demonstrate details about the {\em spatiotemporal tokenizer}, which provides ST features for each ST Unit.
 
\subsection{Unified Spatiotemporal Units}
\label{stunit}
Basic ST elements (in section~\ref{basic_ST_element}) can be integrated into a $T$-length temporal road network $\mathcal{G}_T$, where road network $\mathcal{G}$ captures static spatial features, and current traffic state $\bm{E}_t^{(d)}$ reflects dynamic features of $\mathcal{G}$ at the $t$-th time slice. The structure of $\mathcal{G}_T$ is shown in figure~\ref{STUnit}. Let $\mathcal{G}_t$ is the $t$-th slice of $\mathcal{G}_T$, and each road segment $r_{i,t}$ contains both static and dynamic features, where $r_{i,t} = \left\{\bm{e}_i^{(s)}, \bm{e}_{i,t}^{(d)} \right\}$.



As illustrated in figure~\ref{STUnit}, $\mathcal{G}_T$ can be viewed as a library of basic ST features, and different sampling methods of $\mathcal{G}_T$ lead to various ST data. By combining $\mathcal{G}_T$ with temporal information, we provide a unified structure for ST data, named as the unified STUnit. Specifically, $\bm{U}_{i,t}$ and $\bm{U}_{i,\tau}$ is defined as the STUnit of road segment $r_i$ at timestamp $\tau$ and the $t$-th time slice respectively, \ie
\begin{equation}\label{eq:STU}
  \bm{U}_{i,\tau} = \left\{\;\bm{e}^{(s)}_i, \bm{e}^{(d)}_{i,t}, \bm{\iota}_{\tau} \; \right\} ; \;\;\;
  \bm{U}_{i,t} = \left\{\;\bm{e}^{(s)}_i, \bm{e}^{(d)}_{i,t}, \bm{\iota}_{t} \; \right\},
\end{equation}

Based on the proposed STUnit, we are able to redefine ST data, including trajectory and traffic state series.



\begin{mydef}[STUnit-based Trajectory]
    Given a trajectory with the length of $L$, it can be represented as a sequence of STUnit:
    \begin{equation}\label{eq:trajectory}
      \mathcal{U}_{\mathrm{tr}} = \left( \bm{U}_{\mathrm{tr}_1}, \ldots, \bm{U}_{\mathrm{tr}_l}, \ldots, \bm{U}_{\mathrm{tr}_L} \right).
    \end{equation}
    Here, $\mathrm{tr}_l = \left\{ r_{(l)}, \tau_{(l)} \right\}$, which is the indexes of road segment and timestamp for the $l$-th sample in the given trajectory.
\end{mydef}

% The raw format for a trajectory is a sequence of location coordinates with timestamps. We use map matching algorithms~\cite{yang2018fast} to project the location coordinates onto road segments and the timestamps into time slots. As a result, each trajectory sample corresponds to an ST unit {\small $\bm{U}_{\mathrm{tr}_l}$} in Eq.~\eqref{eq:trajectory}. 

In certain trajectory datasets, the road segments lack traffic states. For these cases, the traffic state { $\bm{e}^{(d)}_{i,t}$} in { $\bm{U}_{\mathrm{tr}_l}$} are set to null.

\begin{mydef}[STUnit-based Traffic State Series]~\label{def:traffic_series}
    The traffic state series for the road segment $r_i$ during the time slice series $\left\{1, \ldots, T\right\}$ is defined as: 
    \begin{equation}\label{eq:traffic_series}
      \mathcal{U}_{\mathrm{ts}}^{i} = \left( \bm{U}_{ts_1}, \ldots, \bm{U}_{ts_t}, \ldots, \bm{U}_{ts_T} \right),
    \end{equation}
    Here, $ts_t = \left\{i, t\right\}$, which is the indexes of road segment and time slice.
    $\mathcal{U}_{\mathrm{ts}}$ denotes traffic state of all $N$ road segments, where $\mathcal{U}_{\mathrm{ts}} = \left\{\mathcal{U}_{\mathrm{ts}}^{1},\cdots,\mathcal{U}_{\mathrm{ts}}^{n},\cdots,\mathcal{U}_{\mathrm{ts}}^{N}\right\}$.
\end{mydef}
Both of the two types of ST data in different modalities are unified in the same format, \ie a sequence of basic ST units. In this way, we can process them using a universal model.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/3_1_model_structure/model_architecture.pdf}
    \caption{\textcolor{red}{The model architecture of \name.}}\label{fig:model_architecture}
\end{figure}


\subsection{The Structure of Spatiotemporal Tokenizer}

As mentioned in section~\ref{stunit}, the temporal road network $\mathcal{G}_T$ is the library of basic ST features. Therefore, we propose a spatiotemporal tokenizer for $\mathcal{G}_T$, encoding basic features into general ST representations.

Since $\mathcal{G}_T$ is composed by static and dynamic features, the sptiotemporal tokenizer comprises three components: a static feature encoder, a dynamic feature encoder, and a fusion encoder.

%The topological relations between road segments can be described as a road network.
% The function of the spatiotemporal (ST) tokenizer is to encode ST units as representation vector-based tokens. We adopt a graph attention network-based (GAT) model to implement the ST tokenizer. First, we adopt the road network data to describe the topological relations between road segments.
% \begin{mydef}[Road Network]
%     A road network is defined as a directed graph $\mathcal{G}=\{R, \bm{A}\}$, where $R = \{r_1, \ldots, r_i, \ldots r_I\}$ is a vertex set corresponding to road segments, and $\bm{A} \in \{0,1\}^{I \times I}$ is an adjacent matrix. The $(i,j)$-th element $a_{i,j} = 1$ refers the segments $r_i$ and $r_{j}$ are connected by a junction.
% \end{mydef}

\paratitle{Static Feature Encoder.} 
The static features comprises the topology structure $\mathcal{G}$ among road segments, and its associated spatial features, denoted as a matrix $\bm{E}^{(s)} = \big( \bm{e}^{(s)}_1, \ldots, \bm{e}^{(s)}_n, \ldots, \bm{e}^{(s)}_N\big)$. 

By taking $\bm{E}^{(s)}$ as input, we employ a $2$-layer graph attention network (GAT) model~\cite{velivckovic2017graph} to generate a representation matrix $\bm{H}^{(s)}$ for the static features of the road network { $\mathcal{G}$} as follows:
\begin{equation}
  \label{eq:GAT1_s}
  \bm{H}^{(s)} = \mathrm{FFN}\left( \mathrm{GAT}_s \big(\bm{E}^{(s)}, \mathcal{G}\big)\right),
\end{equation}
where $\mathrm{GAT}_s(\cdot, \cdot)$ is the GAT model and $\mathrm{FFN}(\cdot)$ is feed forward networks for feature dimensional transformation. Further, {$\bm{H}^{(s)} = \big(\bm{h}^{(s)}_1, \ldots, \bm{h}^{(s)}_n, \ldots, \bm{h}^{(s)}_N\big)$}, where { $\bm{h}^{(s)}_i \in \mathbb{R}^{D_s}$} is the {\em static representation} for the segment $r_i$.

\paratitle{Dynamic Feature Encoder.} 
The dynamic feature is reflected by traffic states. To comprehensively capture the dynamic patterns in data, the dynamic representation of $r_i$ is extracted from its historical traffic state series across a temporal window of length ${T}'$, \ie $\{t-T', \ldots, t-1 \}$.

For the $t$-th time slice, the historical traffic states of $r_i$ is denoted as $\big(\bm{e}^{(d)}_{1,t-T'}\big\| \cdots \big\|\bm{e}^{(d)}_{1,t-1}\big)$, where $\big\|$ is the feature concatenation. Further, the historical traffic states $\mathcal{E}_t^{(d)}$ can be converted as the matrix $\bm{E}^{(d)}_{t, {T}'}$:
% {\small $\bm{E}^{(d)}_t = \big(\bm{e}^{(d)}_{1,t},$ $\ldots,$ $\bm{e}^{(d)}_{I,t}\big)$}. 
\begin{equation}
    \bm{E}^{(d)}_{t,{T}'} = \big[ \big(\bm{e}^{(d)}_{1,t-T'}\big\| \cdots \big\|\bm{e}^{(d)}_{1,t-1}\big),\: \ldots,\: \big( \bm{e}^{(d)}_{N,t-T'}\big\|\cdots \big\| \bm{e}^{(d)}_{N,t-1} \big) \big] \:,
\end{equation}

By taking $\bm{E}^{(d)}_{t,{T}'}$ as input, we adopt another $2$-layer GAT model, denoted as { $\mathrm{GAT}_d(\cdot, \cdot)$} to generate a representation matrix $\bm{H}^{(d)}_t$ for the dynamic features of $\mathcal{R}$ at the $t$-th time slice:
\begin{equation}
  \label{eq:GAT1_s}
  \bm{H}^{(d)}_t = \mathrm{FFN} \left( \mathrm{GAT}_d \left(\bm{E}^{(d)}_{t,{T}'}, \mathcal{G}\right) \right),
\end{equation}
Similarly, where $\mathrm{FFN}(\cdot)$ is to compress the redundant dimension caused by historical temporal window. Further, {$\bm{H}^{(d)}_t = \big(\bm{h}^{(d)}_{1,t}, \ldots, \bm{h}^{(d)}_{n,t}, \ldots, \bm{h}^{(d)}_{N,t}\big)$}, where { $\bm{h}^{(d)}_{i,t} \in \mathbb{R}^{D_d}$} is the {\em dynamic representation} for the road segment $r_i$ at the $t$-th time slice.

\paratitle{Fusion Encoder.} 
The static features $\bm{H}^{(s)}$ and dynamic features $\bm{H}_{t}^{(d)}$ are integrated as $\tilde{\bm{H}}_t \in \mathbb{R}^{N \times D_h}$.
% and let $\bm{h}_{i,t}$ denotes the comprehensive feature of $r_i$ at the $t$-th time slice, and $\bm{h}_{i,t} = \big(\bm{h}^{(s)}_{i}\| \bm{h}^{(d)}_{i,t}\big)$. 
However, road networks is characterized by longer edges and larger scales than typical graphs, posing challenges for GAT in capturing essential long-range spatiotemporal dependencies. 

To address this, we design the fusion encoder based on a cross-attention layer. It uses a set of learnable queries to adaptively capture the long-range spatiotemporal dependencies among $\tilde{\bm{H}}_t$. 

Specifically, the fusion encoder takes $\tilde{\bm{H}}_t$ as both keys and values. $\bm{Q}$ denotes the learnable queries, where $\left | \bm{Q} \right | = N$. The attention weight between $r_{i}$ and $r_{j}$ is calculated as { $\mathrm{ATT}_{ij} = {\alpha_{ij}}\big/{\sum_{j=1}^{N} \alpha_{ij}}$}, where { $\alpha_{ij} = {\bm{q}_i^{\top} \bm{k}_j}\big/{\sqrt{2D_h}}$}. The {\em fused representation} for $r_i$ at the $t$-th time slice is calculated as: 
\begin{equation}\label{}
  \bm{h}_{i,t} = \sum_{j=1}^{N} \mathrm{ATT}_{ij} \cdot (\bm{h}_j^{(s)} \; \big\| \; \bm{h}_{j,t}^{(d)}) \;, 
\end{equation}
where $\bm{q}_i$ is the $t$-th learnable query and $\bm{k}_j$ is the $j$-th key. Further, the whole representations of $\mathcal{G}_T$ is denoted as $\bm{H}_{1,T}$, where $\bm{H}_{1,T} = \left\{\bm{H}_1, \ldots, \bm{H}_t, \ldots, \bm{H}_T \right\}$.

\subsection{Unified Spatiotemporal Input}
\label{unified_input}
Given the STUnit sequence $\mathcal{U} = (\bm{U}_{1}, \ldots, \bm{U}_{l}, \ldots, \bm{U}_{L})$ for an input trajectory (or an input traffic state series), each $\bm{U}_l$ serves as the index of a specific element in $\bm{H}_{1,T}$. The representations of the input is first sampled from $\bm{H}_{1,T}$ through $\mathcal{U}$, and followed by integrating temporal information. The temporal features of $\bm{U}_l$ is denoted as $\bm{\iota}_{\tau_{l}}$. 

A Multilayer Perceptron (MLP) is employed for feature alignment between the spatiotemporal tokenizer and the backbone model. Let $\bm{x}_{l}$ denotes the final representation corresponding to the ST unit $U_l$:  
\begin{equation}\label{eq:st_tokens}
  \bm{x}_{l}^{(\mathrm{st})} = \mathrm{MLP}\Big( \; \bm{h}_{r_{(l)},t_{(l)}} \big\| \; \bm{\iota}_{\tau_l} \Big).
\end{equation} 
where $r_{(l)}$, $t_{(l)}$ is the index of road segment, time slice in $U_l$. As defined in section~\ref{basic_ST_element}, $\bm{\iota}_{\tau_l}$ is the timestamp feature for trajectory while the time slice feature for traffic state. Finally, $\bm{X}^{(\mathrm{st})}$ denotes the unified ST input for a trajectory (or a traffic state series), and $\bm{X}^{(\mathrm{st})} = \big(\bm{x}_{1}^{(\mathrm{st})}, \ldots, \bm{x}_{l}^{(\mathrm{st})}, \ldots, \bm{x}_{L}^{(\mathrm{st})}\big)$. 


==> content/3_3_backbone_model.tex <==
\section{The Backbone Model}
\label{model_structure}
Building a multi-task ST model requires: $1)$ a unified pipeline, and $2)$ a general architecture for hetero ST tasks. 

For the first demand, we propose {\em task-oriented prompts}, enabling \name tackles hetero ST tasks uniformly as sequence modeling.  
For the second, we design our backbone based on LLM (a \backbone~\cite{radford2019language} model), aiming to transfer its general sequence modeling abilities into ST tasks. 

\subsection{Task-Oriented Prompts}
\label{task_oriented_prompts}
Although the spatiotemporal tokenizer unifies ST input data into a sequence format, a unified pipeline for ST tasks remains absent. Firstly, the same ST input may correspond to multiple ST tasks, requiring additional task identifiers. Moreover, Task outputs vary significantly in format and content: regression tasks produce continuous values (e.g., time or traffic state), classification tasks yield discrete road segments, and generation tasks output sequences of road segments.

Therefore, we propose {\em task-oriented prompts}. We first briefly introduce prompts contents. Next, we focus on the structure of prompts, presented as {\em prompt templates}. 
% consisting of three parts: textual instructions as task-specific identifiers, ST data from the spatiotemporal tokenizer, and task placeholders that provide a general format of task outputs.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/prompt_templates/Trajectory Generation.pdf}
    \caption{\textcolor{red}{An Example of Prompt Template.}}
    \label{prompt_example}
\end{figure}



\paratitle{Prompt Contents.}
As \name adopts a LLM as the backbone, thereby task-oriented prompts are combinations of textual data and ST input. Specifically, the prompts consists of three parts: {\em Textual Instructions}, {\em ST Data}, and {\em Task Placeholders}.

\begin{itemize}[leftmargin=*]
\item {\em Textual Instructions} act as task-specific identifiers that guide BIGCity in determining which ST task to tackle. Each ST task is linked to a unique textual instruction. 
The textual instructions are encoded into text token sequences by the LLM backbone’s textual tokenizer, denoted as $\bm{X}^{(\mathrm{txt})}$.
\item {\em ST Data} is originally the ST data to be analyzed, \ie a trajectory or a traffic state series. It is encoded as a sequence by the spatiotemporal tokenizer. As defined in Eq.~\eqref{eq:st_tokens}, ST data is represented as $\bm{X}^{(\mathrm{st})}$.
\item {\em Task Placeholders:} Outputs of ST tasks can be categorized into two types: the discrete classification values and the continuous regression values. Therefore, task placeholders are proposed to indicate output formats. As $\mathrm{[CLS]}$ for classification (prediction, generation tasks) and $\mathrm{[REG]}$ for regression (regression tasks). Task types are defined in section~\ref{problem_statement}). Such placeholder are appended to the end of ST data, with their types and numbers indicating the content and length of outputs respectively. Two learnable vectors, \ie { $\bm{x}^{(\mathrm{clas})}$} and {$\bm{x}^{(\mathrm{reg})}$}, are used to represent $\mathrm{[CLS]}$ and $\mathrm{[REG]}$. In the input, the sequence of task placeholders is denoted as $\bm{X}^{(\mathrm{tsk})}$.
\end{itemize}

\paratitle{Prompt Template.} The prompt template provides a unified structure for prompts across ST tasks. As illustrated in Fig.~\ref{prompt_example}, the template comprises textual instructions, and input (ST data and task placeholders). Details of each module in the template are as follows:

\begin{itemize}[leftmargin=*]
\item {\em Textual instructions} provides two-level identifiers: task-level (``instruction'') and data-level (``supplementary data''). $\bm{1)}$ The ``instruction'' guides model to complete a specific task. For instance, ``generate a time interval on $\mathrm{[REG]}$ based on supplementary data and input'' is the fixed instruction for travel time estimation task. $\bm{2)}$ The ``supplementary data'' is a data-level prompt for a specific input sample. It comprises statistics from training dataset, \ie ``distance'', ``velocity'', and ``density'', with its values vary by input sample. Details are described in section~\ref{sec:prompt_tuning}. Textual instructions are determined before training and inference. In addition, ChatGPT provides reference for designing textual instructions.

\item {\em Input} is a concatenation of ST data and task placeholders, as illustrated in Fig.~\ref{prompt_example}. The {\em input} specifically associates with ST task categories: \; $\bm{1)}$ for classification tasks, ST data is a trajectory, and task placeholder is a single $\mathrm{[CLS]}$; \;
$\bm{2)}$ for regression tasks, ST data is a trajectory or a traffic state series, and task placeholder is a sequence of $\mathrm{[REG]}$; \;
$\bm{3)}$ for generation tasks, ST data is a part of a trajectory, and task placeholder is a sequence of $\mathrm{[CLS]}$. The missing road segments are replaced by $\mathrm{[MASK]}$. 
The number of $\mathrm{[CLS]}$ is related to the number of segments to be generated. 
Detailed examples of {\em input} in each ST task are described in section~\ref{sec:prompt_tuning}. 
\end{itemize}

The final input to the LLM backbone is encapsulated by task-oriented prompts as $\bm{\mathcal{X}}$, where $\bm{\mathcal{X}} = \big(\bm{X}^{(\mathrm{txt})}, \bm{X}^{(\mathrm{st})}, \bm{X}^{(\mathrm{tsk})}\big)$. 


\subsection{The Architecture of Unified Backbone}
Although hetero ST tasks are unified as sequence modeling, designing a unified backbone still faces two issues:
\begin{itemize}[leftmargin=*]
\item Hetero ST tasks leverage different components of ST features, requiring a backbone with high generalization ability.
\item Existing methods rely on task-specific output heads, limited in model structural unification.
\end{itemize}


Figure~\ref{fig:model_architecture} illustrates the structure of the unified backbone. We address the first issue by the proposed tunable LLM backbone. For the second issue, we unified task-specific output modules into two general heads, \ie one head responsible for tasks with discrete outputs and the other for tasks with continuous outputs.

\paratitle{Tunable LLM Backbone.}
\label{sec:tunable_LLM_backbone}

We adopt \backbone~\cite{radford2019language} as our backbone model, and employ Low-Rank Adaptation (LoRA)~\cite{hu2021loralowrankadaptationlarge}. LoRA introduces additional parameters within the transformer block of \backbone, reducing the number of trainable parameters and computational complexity while transferring \backbone’s general sequence modeling ability to new tasks.

As shown in figure~\ref{fig:model_architecture}, LoRA modules are attached to {\em query}, {\em key}, and {\em value} matrices in each block of \backbone. In the training stages, only parameters in LoRA modules are trained while the original parameters of \backbone \ are frozen. For each input sample $\bm{\mathcal{X}}$, the processing in \name is expressed as: 
\begin{equation}\label{eq:LLM}
   \big\{\bm{V}, \bm{Z}\big\} = \mathrm{LLM}\Big(\bm{\mathcal{X}}, \; \bm{\Phi}_{\mathrm{LoRA}}\Big),
\end{equation}
where {$\bm{\Phi}_{\mathrm{LoRA}}$} are learnable parameters for the LoRA modules. The output sequence is divided into two parts: $\bm{Z}$ represents the tokens corresponding to $\bm{X}^{\mathrm{(tsk)}}$, while $\bm{V}$ represents the remaining tokens which corresponds to $\big( \bm{X}^{\mathrm{(txt)}}, \bm{X}^{\mathrm{(st)}} \big)$.

The general task heads only take $\bm{Z}$ as input, and the $k$-th token $\bm{z}_{k}$ in $\bm{Z}$ corresponds to the $k$-th token $\bm{x}^{\mathrm{(tsk)}}_{k}$ in $\bm{X}^{\mathrm{(tsk)}}$.

\paratitle{General Task Head.} Unlike existing methods that use standalone, task-specific output heads, we design a $\mathrm{[CLS]}$ head $H_{\mathrm{CLS}}(\cdot)$ for tasks with discrete outputs and a $\mathrm{[REG]}$ head $H_{\mathrm{REG}}(\cdot)$ for tasks with continuous value, ensuring a more unified model architecture.

The structures of two heads are illustrated in figure~\ref{fig:model_architecture}. We employ individual MLPs, denoted as $\mathrm{MLP}_{ts}$ and $\mathrm{MLP}_{te}(\cdot)$, to regress the continuous values (traffic state and temporal information), respectively. $\mathrm{MLP}_{dis}(\cdot)$ generates the final results of discreet values.

% \textcolor{red}{Although the outputs of hetero ST tasks differ significantly in semantics, they can be concluded into two categories by formats: discrete values (road segments, classification labels) or continuous values (traffic state, timestamps). 
% Specifically, $\bm{v}_{k}$ will be sent to discrete task head if $\bm{x}^{\mathrm{(tsk)}}_{k}$ is $\mathrm{[CLS]}$, while continuous task head otherwise.}

% \begin{itemize}[leftmargin=*]
% \item The {\em representation token} output is a sequence of token vectors { $\bm{V} = \big(\bm{v}_1,$ $\ldots,$ $\bm{v}_K \big)$}, the sequence length $K$ equals to the length of input data token sequence { $\bm{X}^{(\mathrm{st})}$}. We use the last element $\bm{v}_K \in \bm{V}$ as the representation vector for the entire input ST data sequence (a trajectory or a traffic state series).
% \item The {\em result token} output is a sequence of token vectors { $\bm{Z} = \big(\bm{z}_1,$ $\ldots,$ $\bm{z}_{k'},$ $\ldots,$ $\bm{z}_{K'} \big)$}, where the length $K'$  equals to the length of input task token sequence { $\bm{X}^{(\mathrm{tsk})}$}. The element {\em $\bm{z}_{k'} \in \bm{Z}$} corresponds to the $k'$-th task token in { $\bm{X}^{(\mathrm{tsk})}$}.
% \end{itemize}

% Similar as the task tokens, the result tokens also have two types: { $\bm{z}_k^{(\mathrm{clas})}$} corresponding to $[CLAS]$, and { $\bm{z}_k^{(\mathrm{reg})}$} corresponding to $[REG]$. We use MLPs as decoders to convert the result tokens as classification or regression results in different tasks (see Sec.~\ref{sec:training}).




==> content/3_4_training.tex <==
\begin{figure*}[t]
     \centering
     \includegraphics[width=1.0\linewidth]{content/framework_overview.pdf}
     \caption{\textcolor{red}{The hierarchical training strategy of \name.}}
     \label{fig:training_framework}
\end{figure*}


\section{Model Training}
\label{sec:training}
As illustrated in Fig.~\ref{fig:training_framework}, \name employs a two-stage training strategy, including {\em Masked Reconstruction Training} and {\em Task-Oriented Prompt Tuning}. Hetero ST tasks are co-trained through task-oriented prompt tuning, thereby a single model handles diverse tasks without task-specific fine-tuning.


\subsection{Masked Reconstruction Training}
Masked reconstruction training enhances \name’s capacity to learn general ST features, thereby effectively adapt to a specific ST task through task-oriented prompt tuning. 
As illustrated in Fig, \name randomly masks certain samples from $\bm{\mathcal{X}}$ and reconstructs them in $\bm{Z}$. To ensure representation generality, each element in $\bm{Z}$ is supervised from three aspects: static, dynamic, and temporal features.

\paratitle{Input.} In this stage, only ST data and task placeholders participate in training, and $\bm{\mathcal{X}} = \big( \bm{X}^{(\mathrm{st})}, \bm{X}^{(\mathrm{tsk}} \big)$. For each ST data sequence { $\bm{X}^{(\mathrm{st})} = (\bm{x}_{1}, \ldots, \bm{x}_{L})$}, we randomly mask $K$ tokens and replace them by a specific mask token $\mathrm{[MASK]}$. For comprehensive ST representation, each masked token associates with both $\mathrm{[CLS]}$ and $\mathrm{[REG]}$. Therefore, the length of $\bm{X}^{(\mathrm{tsk})}$ is $2K$, and denoted as:
\begin{equation}\label{eq:task_pretrain}
  \bm{X}^{(\mathrm{tsk})} = \left(\big(\bm{x}_1^{(\mathrm{cls})}, \bm{x}_1^{(\mathrm{reg})}\big), \ldots, \big(\bm{x}_K^{(\mathrm{cls})}, \bm{x}_K^{(\mathrm{reg})}\big)\right),
\end{equation}
Subsequently, we take $\bm{Z}$ to generate final results, where each element has a one-to-one correspondence to elements in $\bm{X}^{(\mathrm{tsk})}$ as:
\begin{equation}\label{eq:result_tokens}
\begin{aligned}
  \bm{Z} = \left(\big(\bm{z}_1^{(\mathrm{cls})}, \bm{z}_1^{(\mathrm{reg})}\big), \ldots, \big(\bm{z}_K^{(\mathrm{cls})}, \bm{z}_K^{(\mathrm{reg})}\big)\right),
\end{aligned}
\end{equation}
Further, $\bm{Z}$ is divided into $\bm{Z}^{\mathrm{(cls)}}$ and $\bm{Z}^{\mathrm{(reg)}}$, denoted as: 
\begin{equation}
\label{eq:result_tokens}
  \bm{Z}^{\mathrm{(cls)}} = \big(\bm{z}_1^{(\mathrm{cls})}, \ldots, \bm{z}_K^{(\mathrm{cls})}\big), \; \;
  \bm{Z}^{\mathrm{(reg)}} = \big(\bm{z}_1^{(\mathrm{reg})}, \ldots, \bm{z}_K^{(\mathrm{reg})}\big),
\end{equation}
Then, $H_{\mathrm{CLS}}(\cdot)$ takes $\bm{Z}^{\mathrm{(cls)}}$ as input, and $H_{\mathrm{REG}}(\cdot)$ takes $\bm{Z}^{\mathrm{(reg)}}$ as input. For the $k$-th masked tokens, $\bm{z}_k^{(\mathrm{cls})}$ is supervised by the road segment ID $\bm{y}_k^{(dis)}$, and $\bm{z}_k^{(\mathrm{reg})}$ is supervised by current traffic state $\bm{y}_k^{(ts)}$ and timestamp $\bm{y}_k^{(te)}$. 

\paratitle{Loss Function.} 
We use both Cross-Entropy loss (CE) and Mean Squared Error loss (MSE) as loss function, formulating as follows:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{CE} = L_{CE} & \left( H_{\mathrm{CLS}}(\bm{z}_k^{(\mathrm{cls})}), \bm{y}_k^{(dis)} \right), \\
    \mathcal{L}_{MSE}^{ts} = L_{MSE} & \left(MLP_{ts} \big[ H_{\mathrm{REG}}(\bm{z}_k^{(\mathrm{reg})}) \big], \bm{y}_k^{(dis)} \right), \\ 
    \mathcal{L}_{MSE}^{te} = L_{MSE} & \left(MLP_{te} \big[ H_{\mathrm{REG}}(\bm{z}_k^{(\mathrm{reg})})\big ], \bm{y}_k^{(dis)} \right),
\end{aligned}
\end{equation}
where $L_{CE}$ denotes the cross entropy loss function and $L_{MSE}$ denotes the MSE loss function. The final loss function of masked reconstruction training is denoted as $\mathcal{L}_{MRT}$.
\begin{equation}
\begin{aligned}
\label{pre_loss}
    \mathcal{L}_{MRT} = \frac{1}{K} \textstyle \sum^{K}_{k=1} \big( \alpha \mathcal{L}_{CE} +
     \beta \mathcal{L}_{MSE}^{ts} + \gamma \mathcal{L}_{MSE}^{te} \big).
\end{aligned}
\end{equation}
where $\alpha, \beta, \gamma$ are weight parameters, and $\alpha + \beta + \gamma = 1$.
% \begin{equation}\label{eq:mlp_decoder}
% \begin{aligned}
%     {\bm{y}}_k^{(\mathrm{seg})} = \mathrm{MLP}_s\left(\bm{z}_k^{(\mathrm{clas})}\right), \\
%     {y}_k^{(\mathrm{tim})} = \mathrm{MLP}_t\left(\bm{z}_k^{(\mathrm{reg})}\right), \\
%     {\bm{y}}_k^{(\mathrm{tra})} = \mathrm{MLP}_r\left(\bm{z}_k^{(\mathrm{reg})}\right),
% \end{aligned}
% \end{equation}
% where { ${\bm{y}}_k^{(\mathrm{seg})}$}, { ${y}_k^{(\mathrm{tim})}$}, and { ${\bm{y}}_k^{(\mathrm{tra})}$} are the predicted segment ID, time interval and traffic state for the $k$-th masked sample.


% \subsection{Task-oriented Prompt Tuning}

% \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.8\linewidth]{figure/prompt_template.pdf}
%      \caption{An Example of Prompt Template.}
%      \label{fig:prompt_template}
% \end{figure}

% \subsubsection{Task-tuning Prompts}

% The task-oriented prompt tuning stage is designed to enhance the model's adaptability to various spatial-temporal data analysis tasks. For a given task, the input to our model is a prompt following the template illustrated in Fig.~\ref{fig:prompt_template}. The prompt template contains three parts: {\em Instruction}, {\em Supplementary Data}, and {\em Input Data}.

% \paratitle{Instruction.} The textual instruction prompt specifies the task that our model is required to execute. In the \name model, we define three types of tasks, totaling six tasks:
% ($1$) Two classification tasks, \ie ``trajectory classification'' and ``trajectory next hop prediction''. ($2$) Two regression tasks, \ie ``travel time estimation (TTE)'' and ``traffic state prediction''. ($3$) Two generation tasks, \ie ``trajectory recovery'' and ``trajectory generation''.
% For each task, we construct a set of instructions to prompt our model. For instance, both ``Give me the estimated time of arrival for this trajectory'' and ``Can I walk from home to school in 20 minutes?'' are instructions for the TTE task. To generate sufficient instructions for each task, we use a language model, specifically ChatGPT-4, to understand the function of each task and then generate the instructions. We run the instruction generation multiple times and sort the generated instructions based on their frequency of occurrence. The top 2,000 instructions are adopted for each task.

% \paratitle{Supplementary Data.} The supplementary data prompt provides information in textual format that helps our model complete the data analysis tasks. The supplementary data include {\color{red}x} types, \ie ``Departure Time'', ``Distance'' for trajectory tasks, and {\color{red} ``Weather'' for traffic state series tasks}. We summarize these information from the training datasets and side informant source.

% \paratitle{Input Data.} The input data prompt contain two parts: data tokens and task tokens, of which the format is given in Sec.~\ref{sec:TLM}. For different type of tasks, we give the model different data and task tokens.
% \begin{itemize}[leftmargin=*]
%   \item {\em Classification Tasks:} The data tokens are a trajectory to be classified. The task token is the token vector {\small $\bm{x}^{(\mathrm{clas})}$} corresponding to the task placeholder $[CLAS]$.
%   \item {\em Regression Tasks:} The data tokens are a trajectory or a traffic state series, serving as the regression inputs. The task token is the token vector {\small $\bm{x}^{(\mathrm{reg})}$} corresponding to the task placeholder $[REG]$.
%   \item {\em Generation Tasks:} The data tokens for generation tasks are a trajectory, into which we insert $[MASK]$ tokens at the locations to be generated. For example, in trajectory generation, we provide the first half of a trajectory and its destination location, inserting $[MASK]$ tokens at the intermediate locations to be generated. For trajectory recovery, we insert $N$ $[MASK]$ tokens between adjacent samples in a low sampling rate trajectory, where the number of $N$ is the multiple of the sampling rate to be recovered. Correspondingly, for each $[MASK]$ token, we assign a task token pair {\footnotesize $\big(\bm{x}_k^{(\mathrm{clas})}, \bm{x}_k^{(\mathrm{reg})}\big) $} to compose a task token sequence as Eq.~\eqref{eq:task_pretrain}.
% \end{itemize}


% \subsubsection{Task-tuning Training} Given the trajectories and the traffic state series in a training set, we randomly combine the spatiotemporal data and corresponding supplementary data with the instructions according to the tasks, creating training prompts. Using a training prompt as input, the model outputs a sequence of result tokens {\small $\bm{Z}$} in the form of Eq.~\eqref{eq:result_tokens}. %The result tokens in {\small $\bm{Z}$} have a one-to-one correspondence with the input task tokens.
% We use MLP models in Eq.~\eqref{eq:mlp_decoder} to decode the result tokens. Specifically, we use {\small ${\bm{y}} = \mathrm{MLP}_s\big(\bm{x}_k^{(\mathrm{clas})}\big)$} to generate results for the trajectory classification and next hop prediction tasks, use {\small ${\bm{y}} =\mathrm{MLP}_t\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for the TTE task, and use {\small ${\bm{y}} =\mathrm{MLP}_r\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for traffic state prediction. For the trajectory generation tasks, we use the results from all three models in Eq.~\eqref{eq:mlp_decoder} to form the trajectory samples to be generated. Finally, the ground truths of ${\bm{y}}$ are used as supervised labels to tune parameters in the LoRA models and MLP decoders. 



\subsection{Task-Oriented Prompt Tuning}
\label{sec:prompt_tuning}
In this stage, \name is co-trained on hetero ST tasks, as task-oriented prompts provide a unified input data format. Therefore, a single multi-task model is able to switch tasks by following task-oriented prompts. 

\paratitle{Input.} 
In section~\ref{task_oriented_prompts}, we briefly introduce prompt contents and templates, where we denote that textual instructions and task placeholders vary with task type. 

In the textual instruction, the ``instruction'' varies with task type and ``supplementary data'' vary with input sample. 
Specifically, the concrete contents of ``supplementary data'' are listed as Tab.~\ref{tab:task_types}.



Detailed contents of each ST task are described as follows:
\begin{itemize}[leftmargin=*]
\item {\em Classification Tasks} consists of next hop prediction (in Fig.~\ref{next_hop_template}) and trajectory classification (in Fig.~\ref{next_hop_template}). The $\bm{X}^{(\mathrm{tsk})}$ is a single $\mathrm{[CLS]}$. 
\item {\em Regression Tasks} comprises ETA (in Fig.~\ref{ETA}) and traffic state prediction (in Fig.~\ref{traffic_state}). For a $2L$-length input, the ETA task outputs temporal information for each token, thereby $\bm{X}^{(\mathrm{tsk})}$ is a $2L$-length sequence of $\mathrm{[REG]}$. In contrast, traffic state prediction uses the first half of the input to predict the traffic state of the second half, resulting in an $L$-length sequence of $\mathrm{[REG]}$.
\item {\em Generation Tasks} comprise trajectory recovery (in Fig.~\ref{traj_recovery}), where certain parts of $\bm{X}^{(\mathrm{st})}$ are replaced by $\mathrm{[MASK]}$. Each $\mathrm{[MASK]}$ represents an individual missing token. The $\bm{X}^{(\mathrm{tsk})}$ is a sequence of $\mathrm{[CLS]}$ with the same number of $\mathrm{[MASK]}$. The missing parts are recovered in $\mathrm{[CLS]}$.
\end{itemize}


\paratitle{Loss Function.} We co-trained \name on hetero ST tasks with the same output formats in masked reconstruction training. Thus, the loss function in this stage is similar to Eq.~\ref{pre_loss}.
\begin{equation}
\begin{aligned}
\label{prompt_tuning}
    \mathcal{L}_{PT} = \frac{1}{K} \textstyle \sum^{K}_{k=1} \big( \alpha \mathcal{L}_{CE} +
     \beta \mathcal{L}_{MSE}^{ts} + \gamma \mathcal{L}_{MSE}^{te} \big).
\end{aligned}
\end{equation}
where $\mathcal{L}_{PT}$ denotes the loss of task-oriented prompt tuning. $\alpha, \beta, \gamma$ are weight parameters, and $\alpha + \beta + \gamma = 1$. Specifically, comparison tasks are commonly used to evaluate the representation quality. Following the general setting like ~\cite{jiang2023self,ma2024more}, we did not train comparison tasks in this stage.

% \subsubsection{Task-tuning Training} Given the trajectories and the traffic state series in a training set, we combine the spatiotemporal data with corresponding supplements and instructions according to the tasks, creating training prompts. Using a training prompt as input, the model outputs a sequence of result tokens { $\bm{Z}$} in the form of Eq.~\eqref{eq:result_tokens}. 
% We use MLP models in Eq.~\eqref{eq:mlp_decoder} to decode the result tokens. Specifically, we use { ${\bm{y}} = \mathrm{MLP}_s\big(\bm{x}_k^{(\mathrm{clas})}\big)$} to generate results for the trajectory classification and next hop prediction tasks, use { ${\bm{y}} =\mathrm{MLP}_t\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for the TTE task, and use { ${\bm{y}} =\mathrm{MLP}_r\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for traffic state prediction. For the trajectory generation tasks, we use the results from ${\small \mathrm{MLP}_s\big(\bm{x}_k^{(\mathrm{clas})} \big)}$
% % all three models in Eq.~\eqref{eq:mlp_decoder} 
% to form the road segments to be generated. Finally, the ground truths of ${\bm{y}}$ are used as supervised labels to tune parameters in the LoRA models and MLP decoders.  





==> content/8_prototype_system.tex <==
\section{A Prototype System}
We aim to integrate \name into applications such as Huawei Navigation and Huawei Maps to enhance their intelligence and functionality. To validate this, we developed a prototype system. As shown in Figure~\ref{fig:proto}, it comprises four main components: the display interface, input module, prompt selection, and input instructions. The input instructions specify the required data types and input formats for \name. These include a sequence of road segment indices, timestamps in sequence format, the city, the corresponding time slice, and the task-specific prompt. In the display interface, \name dynamically generates task results based on the selected prompt and visualizes them on a map. Figure~\ref{fig:proto} takes trajectory recovery as a showcase.
\vspace{-0.2cm}
\begin{figure}[t]
     \centering
     \includegraphics[width=0.85\columnwidth, page=1]{figure/4_experiment/proto.jpg}
     \caption{The trajectory recovery results on prototype system.}
     \label{fig:proto}
     \vspace{-0.5cm}
\end{figure}



==> content/wang_version/3_5_training_2.tex <==
\section{Model Training}
\label{sec:training}

%\setlength{\belowcaptionskip}{-0.25cm}

The \name model adopts a progressive training strategy, including three stages: {\em trajectory reconstruction pre-training} (pre-training), {\em task-oriented prompt tuning} (task-tuning), and {generative reinforcement learning} (GRL). The training stages are illustrated in Fig.~\ref{fig:training_framework}.

\subsection{Trajectory Reconstruction Pretraining}

The pre-training stage randomly masks certain samples from a trajectory and trains \name to reconstruct these masked samples. Specifically, given a trajectory in the format of data token sequence, denoted as { $\bm{X}^{(\mathrm{st})} = (\bm{x}_{tr_1}, \ldots, \bm{x}_{tr_L})$}, we randomly select $K$ samples and replace them as the mask token $[MASK]$. For the $k$-th masked data token, we assign two task tokens, denoted as { $\bm{x}_k^{(\mathrm{clas})}$} and { $\bm{x}_k^{(\mathrm{reg})}$}. Corresponding to the $K$ masked samples in the trajectory, we have a task token sequence as the inputs of
\begin{equation}\label{eq:task_pretrain}\footnotesize
  \bm{X}^{(\mathrm{tsk})} = \left(\big(\bm{x}_1^{(\mathrm{clas})}, \bm{x}_1^{(\mathrm{reg})}\big), \ldots, \big(\bm{x}_k^{(\mathrm{clas})}, \bm{x}_k^{(\mathrm{reg})}\big), \ldots, \big(\bm{x}_K^{(\mathrm{clas})}, \bm{x}_K^{(\mathrm{reg})}\big)\right).
\end{equation}
We use both the trajectory data tokens { $\bm{X}^{(\mathrm{st})}$} with masked samples and the task token sequence { $\bm{X}^{(\mathrm{tsk})}$} as inputs of our model. The outputs are a sequence of result tokens in $\bm{Z}$ that have a one-to-one correspondence to the task tokens in { $\bm{X}^{(\mathrm{tsk})}$}, \ie
\begin{equation}\label{eq:result_tokens}\small
  \bm{Z} = \left(\big(\bm{z}_1^{(\mathrm{clas})}, \bm{z}_1^{(\mathrm{reg})}\big), \ldots, \big(\bm{z}_k^{(\mathrm{clas})}, \bm{z}_k^{(\mathrm{reg})}\big), \ldots, \big(\bm{z}_K^{(\mathrm{clas})}, \bm{z}_K^{(\mathrm{reg})}\big)\right).
\end{equation}
For the $k$-th masked trajectory sample, we a MLP model, denoted as $\mathrm{MLP}_s(\cdot)$, to decode the classification result token { $\bm{z}_k^{(\mathrm{clas})}$} as the segment ID, and use two MLP models, \ie $\mathrm{MLP}_t(\cdot)$ and $\mathrm{MLP}_r(\cdot)$, to decode the regression result token {\ $\bm{z}_k^{(\mathrm{reg})}$} as the timestemp and the traffic state, \ie
\begin{equation}\label{eq:mlp_decoder}
\begin{aligned}
    {\bm{y}}_k^{(\mathrm{seg})} = \mathrm{MLP}_s\left(\bm{z}_k^{(\mathrm{clas})}\right), \\
    {y}_k^{(\mathrm{tim})} = \mathrm{MLP}_t\left(\bm{z}_k^{(\mathrm{reg})}\right), \\
    {\bm{y}}_k^{(\mathrm{tra})} = \mathrm{MLP}_r\left(\bm{z}_k^{(\mathrm{reg})}\right),
\end{aligned}
\end{equation}
where { ${\bm{y}}_k^{(\mathrm{seg})}$}, { ${y}_k^{(\mathrm{tim})}$}, and { ${\bm{y}}_k^{(\mathrm{tra})}$} are the predicted segment ID, time interval and traffic state for the $k$-th masked sample.

Finally, we optimize the parameters in ST tokenizer, the LoRA modules and the MLP decoders by minimizing the errors between { ${\bm{y}}_k^{(\mathrm{seg})}$}, { ${y}_k^{(\mathrm{tim})}$}, { ${\bm{y}}_k^{(\mathrm{tra})}$} and their ground truth for all trajectories in the training set. We use the cross entropy loss for the classification task while the mean square error (MSE) loss for the regression tasks.

% \subsection{Task-oriented Prompt Tuning}

% \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.8\linewidth]{figure/prompt_template.pdf}
%      \caption{An Example of Prompt Template.}
%      \label{fig:prompt_template}
% \end{figure}

% \subsubsection{Task-tuning Prompts}

% The task-oriented prompt tuning stage is designed to enhance the model's adaptability to various spatial-temporal data analysis tasks. For a given task, the input to our model is a prompt following the template illustrated in Fig.~\ref{fig:prompt_template}. The prompt template contains three parts: {\em Instruction}, {\em Supplementary Data}, and {\em Input Data}.

% \paratitle{Instruction.} The textual instruction prompt specifies the task that our model is required to execute. In the \name model, we define three types of tasks, totaling six tasks:
% ($1$) Two classification tasks, \ie ``trajectory classification'' and ``trajectory next hop prediction''. ($2$) Two regression tasks, \ie ``travel time estimation (TTE)'' and ``traffic state prediction''. ($3$) Two generation tasks, \ie ``trajectory recovery'' and ``trajectory generation''.
% For each task, we construct a set of instructions to prompt our model. For instance, both ``Give me the estimated time of arrival for this trajectory'' and ``Can I walk from home to school in 20 minutes?'' are instructions for the TTE task. To generate sufficient instructions for each task, we use a language model, specifically ChatGPT-4, to understand the function of each task and then generate the instructions. We run the instruction generation multiple times and sort the generated instructions based on their frequency of occurrence. The top 2,000 instructions are adopted for each task.

% \paratitle{Supplementary Data.} The supplementary data prompt provides information in textual format that helps our model complete the data analysis tasks. The supplementary data include {\color{red}x} types, \ie ``Departure Time'', ``Distance'' for trajectory tasks, and {\color{red} ``Weather'' for traffic state series tasks}. We summarize these information from the training datasets and side informant source.

% \paratitle{Input Data.} The input data prompt contain two parts: data tokens and task tokens, of which the format is given in Sec.~\ref{sec:TLM}. For different type of tasks, we give the model different data and task tokens.
% \begin{itemize}[leftmargin=*]
%   \item {\em Classification Tasks:} The data tokens are a trajectory to be classified. The task token is the token vector {\small $\bm{x}^{(\mathrm{clas})}$} corresponding to the task placeholder $[CLAS]$.
%   \item {\em Regression Tasks:} The data tokens are a trajectory or a traffic state series, serving as the regression inputs. The task token is the token vector {\small $\bm{x}^{(\mathrm{reg})}$} corresponding to the task placeholder $[REG]$.
%   \item {\em Generation Tasks:} The data tokens for generation tasks are a trajectory, into which we insert $[MASK]$ tokens at the locations to be generated. For example, in trajectory generation, we provide the first half of a trajectory and its destination location, inserting $[MASK]$ tokens at the intermediate locations to be generated. For trajectory recovery, we insert $N$ $[MASK]$ tokens between adjacent samples in a low sampling rate trajectory, where the number of $N$ is the multiple of the sampling rate to be recovered. Correspondingly, for each $[MASK]$ token, we assign a task token pair {\footnotesize $\big(\bm{x}_k^{(\mathrm{clas})}, \bm{x}_k^{(\mathrm{reg})}\big) $} to compose a task token sequence as Eq.~\eqref{eq:task_pretrain}.
% \end{itemize}


% \subsubsection{Task-tuning Training} Given the trajectories and the traffic state series in a training set, we randomly combine the spatiotemporal data and corresponding supplementary data with the instructions according to the tasks, creating training prompts. Using a training prompt as input, the model outputs a sequence of result tokens {\small $\bm{Z}$} in the form of Eq.~\eqref{eq:result_tokens}. %The result tokens in {\small $\bm{Z}$} have a one-to-one correspondence with the input task tokens.
% We use MLP models in Eq.~\eqref{eq:mlp_decoder} to decode the result tokens. Specifically, we use {\small ${\bm{y}} = \mathrm{MLP}_s\big(\bm{x}_k^{(\mathrm{clas})}\big)$} to generate results for the trajectory classification and next hop prediction tasks, use {\small ${\bm{y}} =\mathrm{MLP}_t\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for the TTE task, and use {\small ${\bm{y}} =\mathrm{MLP}_r\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for traffic state prediction. For the trajectory generation tasks, we use the results from all three models in Eq.~\eqref{eq:mlp_decoder} to form the trajectory samples to be generated. Finally, the ground truths of ${\bm{y}}$ are used as supervised labels to tune parameters in the LoRA models and MLP decoders.

\subsection{Task-oriented Prompt Tuning}

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.9\linewidth]{figure/prompt_templates/Trajectory Generation.pdf}
%    \caption{An Example of Prompt Template.}
%    \label{prompt_example}
%\end{figure}

\subsubsection{Task-tuning Prompts}

The task-oriented prompt tuning stage is designed to enhance the model's adaptability to various spatial-temporal data analysis tasks. For a given task, the input to our model is a prompt following the template illustrated in Fig.~\ref{prompt_example}. The prompt template contains three parts: {\em Instruction}, {\em Supplement}, and {\em Input}.

\paratitle{Instruction.} The textual instruction prompt specifies the task that our model is required to execute. In the \name model, instruction is used in three types of tasks, totaling six specific tasks:
($1$) Two classification tasks, \ie ``trajectory classification'' and ``trajectory next hop prediction''. ($2$) Three regression tasks, \ie ``travel time estimation (TTE)'' and ``traffic state prediction in one or multi-steps''. ($3$) Two generation tasks, \ie ``trajectory recovery'' and ``trajectory generation''.
For each task, we construct a set of instructions to prompt our model. For instance, both ``Give me the estimated time of arrival for this trajectory'' and ``Can I walk from home to school in 20 minutes?'' can be the instructions for the TTE task. To generate sufficient instructions for each task, we use a language model, specifically ChatGPT, to understand the function of each task and then generate the instructions. By testing multiple times, we selected the most effective instruction formats as shown in the Fig.~\ref{prompt_example}.

\paratitle{Supplement.} The supplement prompt provides information in textual format as the supplementary data of the instruction, helping our model complete the data analysis tasks. The supplement consists of three types: ``Departure Time'', ``Distance'' , and 'velocity' for trajectory tasks. We summarize these information from the training datasets. All supplements provides approximate ranges rather than precise values. The three types of supplement may not always be present simultaneously. We will remove those that could potentially lead to label leakage depends on the task requirements. For instance, in the TTE task, the supplement 'departure time' is excluded.

\paratitle{Input.} The input data prompt contain two parts: data tokens and task tokens, of which the format is given in Sec.~\ref{sec:TLM}. For different type of tasks, we give the model different data and task tokens.
\begin{itemize}[leftmargin=*]
  \item {\em Classification Tasks:} The data tokens are a trajectory to be classified. The task token is the token vector { $\bm{x}^{(\mathrm{clas})}$} corresponding to the task placeholder $[CLAS]$.
  \item {\em Regression Tasks:} The data tokens are a trajectory or a traffic state series, serving as the regression inputs. The task token is the token vector { $\bm{x}^{(\mathrm{reg})}$} corresponding to the task placeholder $[REG]$.
  \item {\em Generation Tasks:} The data tokens for generation tasks are a trajectory, into which we insert $[MASK]$ tokens at the locations to be generated. For example, in trajectory generation, we provide the first few segments of a trajectory and its destination location, inserting $[MASK]$ tokens to the intermediate locations to be generated. For trajectory recovery, we insert $N$ $[MASK]$ tokens between adjacent samples in a low sampling rate trajectory, where the number of $N$ is the multiple of the sampling rate to be recovered.
  % Correspondingly, for each $[MASK]$ token, we assign a task token pair {\footnotesize $\big(\bm{x}_k^{(\mathrm{clas})}, \bm{x}_k^{(\mathrm{reg})\big) $} to compose a task token sequence as Eq.~\eqref{eq:task_pretrain}.
  Correspondingly, for each $[MASK]$ token, we assign a task token pair { $\big(\bm{x}_k^{(\mathrm{clas})} \big) $} to compose a task token sequence as Eq.~\eqref{eq:task_pretrain}. The final length of the output depends on when \name generates the specific end tokens, denoted as $[EOS]$.
\end{itemize}

\subsubsection{Task-tuning Training} Given the trajectories and the traffic state series in a training set, we combine the spatiotemporal data with corresponding supplements and instructions according to the tasks, creating training prompts. Using a training prompt as input, the model outputs a sequence of result tokens { $\bm{Z}$} in the form of Eq.~\eqref{eq:result_tokens}.
We use MLP models in Eq.~\eqref{eq:mlp_decoder} to decode the result tokens. Specifically, we use { ${\bm{y}} = \mathrm{MLP}_s\big(\bm{x}_k^{(\mathrm{clas})}\big)$} to generate results for the trajectory classification and next hop prediction tasks, use { ${\bm{y}} =\mathrm{MLP}_t\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for the TTE task, and use { ${\bm{y}} =\mathrm{MLP}_r\big(\bm{x}_k^{(\mathrm{reg})}\big)$} to generate results for traffic state prediction. For the trajectory generation tasks, we use the results from ${\small \mathrm{MLP}_s\big(\bm{x}_k^{(\mathrm{clas})} \big)}$
% all three models in Eq.~\eqref{eq:mlp_decoder}
to form the road segments to be generated. Finally, the ground truths of ${\bm{y}}$ are used as supervised labels to tune parameters in the LoRA models and MLP decoders.


